Balancing-based model reduction for output-constrained optimal control of switched linear systems

We develop a balanced-truncation (BT) framework for model-order reduction of optimal control problems governed by switched linear systems, with quadratic tracking costs, convex input constraints, and Moreau--Yosida-regularized output constraints. For general Petrov--Galerkin reduced models, we derive an a posteriori bound for the error in the optimal value function, and combine it with BT-based estimates of the dynamical-system reduction error. We show that BT preserves the duality structure underlying the first-order optimality conditions, making first-reduce-then-optimize and first-optimize-then-reduce equivalent. Consequently, reducing the forward system also reduces the associated optimality system, leading to a certified, online-efficient, and online-adaptive approximation of the parameterized solution operator. The reduced model can therefore be reused across different regularization parameters, constraint sets, switching signals, and reference trajectories.

==> siam-xetex-compat.tex <==
% XeTeX/Tectonic compatibility for the unchanged official SIAM class.
% breakurl's PostScript setup is inappropriate for the hxetex driver.
% Select its PDF-compatible URL aliases only during package loading.
\RequirePackage{ifpdf}
\AddToHook{package/breakurl/before}{%
  \let\siamsavedifpdf\ifpdf
  \let\ifpdf\iftrue}
\AddToHook{package/breakurl/after}{%
  \let\ifpdf\siamsavedifpdf}

